On the Limits of HARQ Prediction for Short Deterministic Codes with Error Detection in Memoryless Channels (Extended Version with Proofs)

We provide a mathematical framework to analyze the limits of Hybrid Automatic Repeat reQuest (HARQ) and derive analytical expressions for the most powerful test for estimating the decodability under maximum-likelihood decoding and $t$-error decoding. Furthermore, we numerically approximate the most powerful test for sum-product decoding. We compare the performance of previously studied HARQ prediction schemes and show that none of the state-of-the-art HARQ prediction is most powerful to estimate the decodability of a partially received signal vector under maximum-likelihood decoding and sum-product decoding. Furthermore, we demonstrate that decoding in general is suboptimal for predicting the decodability.

==> acro.definitions.tex <==
% --------------------------------------------------------------------------
% the ACRO package
% 
%   Typeset Acronyms
% 
% --------------------------------------------------------------------------
% Clemens Niederberger
% Web:    https://bitbucket.org/cgnieder/acro/
% E-Mail: contact@mychemistry.eu
% --------------------------------------------------------------------------
% Copyright 2011--2020 Clemens Niederberger
% 
% This work may be distributed and/or modified under the
% conditions of the LaTeX Project Public License, either version 1.3
% of this license or (at your option) any later version.
% The latest version of this license is in
%   http://www.latex-project.org/lppl.txt
% and version 1.3 or later is part of all distributions of LaTeX
% version 2005/12/01 or later.
% 
% This work has the LPPL maintenance status `maintained'.
% 
% The Current Maintainer of this work is Clemens Niederberger.
% --------------------------------------------------------------------------
% The acro package consists of the files
% - acro.sty, acro.definitions.tex, acro.cfg
% - acro-manual.tex, acro-manual.pdf, acro-manual.cls
% - acro.history, README
% --------------------------------------------------------------------------
% If you have any ideas, questions, suggestions or bugs to report, please
% feel free to contact me.
% --------------------------------------------------------------------------
\ExplSyntaxOn

% document commands:
\NewDocumentCommand \DeclareAcronym {mm}
  { \acro_declare_acronym:nn {#1} {#2} }

\NewDocumentCommand \acsetup { m }
  {
    \tl_if_blank:nF {#1}
      { \keys_set:nn {acro} {#1} }
    \ignorespaces
  }

\NewDocumentCommand \ProvideAcroEnding {mmm}
  { \acro_provide_ending:nnn {#1} {#2} {#3} }

\NewDocumentCommand \AcroRegisterTrailing {mm}
  { \acro_register_trailing_token:Nn #1 {#2} }

\NewDocumentCommand \DeclareAcroTranslation {mm}
  { \acro_declare_translation:nn {#1} {#2} }

\DeclareExpandableDocumentCommand \acifused { m }
  { \acro_if_acronym_used:nTF {#1} }

\NewDocumentCommand \acresetall {}
  { \acro_reset_all: }

\NewDocumentCommand \acuseall {}
  { \acro_mark_all_as_used: }

\NewDocumentCommand \acreset { > { \SplitList {,} } m }
  { \ProcessList {#1} { \acro_reset:n } \ignorespaces }

\NewDocumentCommand \acuse { > { \SplitList {,} } m }
  { \ProcessList {#1} { \acro_mark_as_used:n } \ignorespaces }

\NewDocumentCommand \acfirstupper {m}
  { \acro_first_upper_case:n {#1} }

\NewExpandableDocumentCommand \aciffirst {+m+m}
  { \bool_if:NTF \l__acro_first_instance_bool {#1} {#2} }

\NewDocumentCommand \acdot   {} { \acro_dot: }
\NewDocumentCommand \acspace {} { \acro_space: }

\NewDocumentCommand \acbarrier {}
  { \acro_barrier: }

\NewDocumentCommand \acswitchoff {}
  { \acro_switch_off: }

\NewDocumentCommand \acswitchon {}
  { \acro_switch_on: }

\NewDocumentCommand \printacronyms { O{} }
  { \acro_print_acronyms:n {#1} }

% --------------------------------------------------------------------------
% styles
% #1: name
% #2: template
% #3: settings
\NewDocumentCommand \DeclareAcroFirstStyle {mmm}
  { \acro_declare_first_style:nnn {#1} {#2} {#3} }

\NewDocumentCommand \DeclareAcroExtraStyle {mmm}
  { \acro_declare_extra_style:nnn {#1} {#2} {#3} }

\NewDocumentCommand \DeclareAcroPageStyle {mmm}
  { \acro_declare_page_style:nnn {#1} {#2} {#3} }

\NewDocumentCommand \DeclareAcroListHeading {mm}
  { \acro_declare_list_heading:nn {#1} {#2} }

\NewDocumentCommand \DeclareAcroListStyle {mmm}
  { \acro_declare_list_style:nnn {#1} {#2} {#3} }

% --------------------------------------------------------------------------
% endings:
\ProvideAcroEnding {plural} {s} {s}

% --------------------------------------------------------------------------
% use acronyms:
% automatic:
\NewAcroCommand \ac
  { \acro_use:n {#1} }

\NewAcroCommand \Ac
  {
    \acro_first_upper:
    \acro_use:n {#1}
  }

\NewAcroCommand \iac
  {
    \acro_indefinite:
    \acro_use:n {#1}
  }

\NewAcroCommand \Iac
  {
    \acro_first_upper:
    \acro_indefinite:
    \acro_use:n {#1}
  }

\NewAcroCommand \acp
  {
    \acro_plural:
    \acro_use:n {#1}
  }

\NewAcroCommand \Acp
  {
    \acro_plural:
    \acro_first_upper:
    \acro_use:n {#1}
  }

\NewAcroCommand \acsingle
  {
    \acro_get:n {#1}
    \acro_single:n {#1}
  }

\NewAcroCommand \acpsingle
  {
    \acro_get:n {#1}
    \acro_plural:
    \acro_single:n {#1}
  }

\NewAcroCommand \Acsingle
  {
    \acro_get:n {#1}
    \acro_first_upper:
    \acro_single:n {#1}
  }

\NewAcroCommand \Acpsingle
  {
    \acro_get:n {#1}
    \acro_first_upper:
    \acro_plural:
    \acro_single:n {#1}
  }

% short:
\NewAcroCommand \acs
  { \acro_short:n {#1} }

\NewAcroCommand \Acs
  {
    \acro_first_upper:
    \acro_short:n {#1}
  }

\NewAcroCommand \iacs
  {
    \acro_indefinite:
    \acro_short:n {#1}
  }

\NewAcroCommand \Iacs
  {
    \acro_first_upper:
    \acro_indefinite:
    \acro_short:n {#1}
  }

\NewAcroCommand \acsp
  {
    \acro_plural:
    \acro_short:n {#1}
  }

\NewAcroCommand \Acsp
  {
    \acro_first_upper:
    \acro_plural:
    \acro_short:n {#1}
  }

% alt:
\NewAcroCommand \aca
  { \acro_alt:n {#1} }

\NewAcroCommand \Aca
  {
    \acro_first_upper:
    \acro_alt:n {#1}
  }
  
\NewAcroCommand \iaca
  {
    \acro_indefinite:
    \acro_alt:n {#1}
  }

\NewAcroCommand \Iaca
  {
    \acro_first_upper:
    \acro_indefinite:
    \acro_alt:n {#1}
  }

\NewAcroCommand \acap
  {
    \acro_plural:
    \acro_alt:n {#1}
  }

\NewAcroCommand \Acap
  {
    \acro_first_upper:
    \acro_plural:
    \acro_alt:n {#1}
  }

% long:
\NewAcroCommand \acl
  { \acro_long:n {#1} }

\NewAcroCommand \Acl
  {
    \acro_first_upper:
    \acro_long:n {#1}
  }

\NewAcroCommand \iacl
  {
    \acro_indefinite:
    \acro_long:n {#1}
  }

\NewAcroCommand \Iacl
  {
    \acro_first_upper:
    \acro_indefinite:
    \acro_long:n {#1}
  }

\NewAcroCommand \aclp
  {
    \acro_plural:
    \acro_long:n {#1}
  }

\NewAcroCommand \Aclp
  {
    \acro_plural:
    \acro_first_upper:
    \acro_long:n {#1}
  }

% first:
\NewAcroCommand \acf
  { \acro_first:n {#1} }

\NewAcroCommand \Acf
  {
    \acro_first_upper:
    \acro_first:n {#1}
  }

\NewAcroCommand \iacf
  {
    \acro_indefinite:
    \acro_first:n {#1}
  }

\NewAcroCommand \Iacf
  {
    \acro_first_upper:
    \acro_indefinite:
    \acro_first:n {#1}
  }

\NewAcroCommand \acfp
  {
    \acro_plural:
    \acro_first:n {#1}
  }

\NewAcroCommand \Acfp
  {
    \acro_plural:
    \acro_first_upper:
    \acro_first:n {#1}
  }

% first-like:
\NewPseudoAcroCommand \acflike
  { \acro_first_like:nn {#1} {#2} }

\NewPseudoAcroCommand \iacflike
  {
    \acro_indefinite:
    \acro_first_like:nn {#1} {#2}
  }

\NewPseudoAcroCommand \Iacflike
  {
    \acro_first_upper:
    \acro_indefinite:
    \acro_first_like:nn {#1} {#2}
  }

\NewPseudoAcroCommand \acfplike
  {
    \acro_plural:
    \acro_first_like:nn {#1} {#2}
  }

% --------------------------------------------------------------------------
% first appearance styles:
\DeclareAcroFirstStyle {default} {inline}
  { }

\DeclareAcroFirstStyle {reversed} {inline}
  { reversed = true }

\DeclareAcroFirstStyle {short} {inline}
  {
    only-short = true ,
    brackets = false
  }

\DeclareAcroFirstStyle {long} {inline}
  {
    only-long = true ,
    brackets = false
  }

\DeclareAcroFirstStyle {square} {inline}
  { brackets-type = [] }

\DeclareAcroFirstStyle {plain} {inline}
  {
    brackets = false ,
    between = --
  }

\DeclareAcroFirstStyle {plain-reversed} {inline}
  { 
    brackets = false ,
    between = -- ,
    reversed = true
  }

\DeclareAcroFirstStyle {footnote} {note}
  { }

\DeclareAcroFirstStyle {footnote-reversed} {note}
  { reversed = true }

\DeclareAcroFirstStyle {sidenote} {note}
  { note-command = \sidenote {#1} }

\DeclareAcroFirstStyle {sidenote-reversed} {note}
  {
    note-command = \sidenote {#1} ,
    reversed     = true
  }

\DeclareAcroFirstStyle {empty} {note}
  { use-note = false }

% --------------------------------------------------------------------------
% extra info appearance styles:
\DeclareAcroExtraStyle {default} {inline}
  {
    brackets     = false ,
    punct        = true ,
    punct-symbol = .
  }

\DeclareAcroExtraStyle {plain} {inline}
  {
    brackets     = false ,
    punct        = true ,
    punct-symbol =
  }

\DeclareAcroExtraStyle {paren} {inline}
  {
    brackets     = true ,
    punct        = true ,
    punct-symbol =
  }

\DeclareAcroExtraStyle {bracket} {inline}
  {
    brackets      = true ,
    punct         = true ,
    punct-symbol  = ,
    brackets-type = []
  }

\DeclareAcroExtraStyle {comma} {inline}
  {
    punct         = true,
    punct-symbol  = {,} ,
    brackets      = false
  }

% --------------------------------------------------------------------------
% page number appearance styles:
\DeclareAcroPageStyle {default} {inline}
  {
    punct = true ,
    punct-symbol = .
  }
  
\DeclareAcroPageStyle {plain}   {inline}
  { punct = false }

\DeclareAcroPageStyle {comma}   {inline}
  { punct = true }

\DeclareAcroPageStyle {paren}   {inline}
  {
    brackets=true ,
    punct-symbol = ~
  }

\DeclareAcroPageStyle {none}    {inline}
  { display = false }

% --------------------------------------------------------------------------
% list heading styles:
\DeclareAcroListHeading {part}           {\part}
\DeclareAcroListHeading {part*}          {\part*}
\DeclareAcroListHeading {chapter}        {\chapter}
\DeclareAcroListHeading {chapter*}       {\chapter*}
\DeclareAcroListHeading {addchap}        {\addchap}
\DeclareAcroListHeading {section}        {\section}
\DeclareAcroListHeading {section*}       {\section*}
\DeclareAcroListHeading {addsec}         {\addsec}
\DeclareAcroListHeading {subsection}     {\subsection}
\DeclareAcroListHeading {subsection*}    {\subsection*}
\DeclareAcroListHeading {subsubsection}  {\subsubsection}
\DeclareAcroListHeading {subsubsection*} {\subsubsection*}
\DeclareAcroListHeading {none}           {\use_none:n}

% --------------------------------------------------------------------------
% list styles:
\DeclareAcroListStyle {description} {list}
  { }

\DeclareAcroListStyle {toc} {list-of}
  { }

\DeclareAcroListStyle {lof} {list-of}
  { style = lof }

\DeclareAcroListStyle {tabular} {table}
  { table = tabular }

\DeclareAcroListStyle {longtable} {table}
  { table = longtable }

\DeclareAcroListStyle {extra-tabular} {extra-table}
  { table = tabular }

\DeclareAcroListStyle {extra-longtable} {extra-table}
  { table = longtable }

\DeclareAcroListStyle {extra-tabular-rev} {extra-table}
  {
    table   = tabular ,
    reverse = true
  }

\DeclareAcroListStyle {extra-longtable-rev} {extra-table}
  {
    table   = longtable ,
    reverse = true
  }

% --------------------------------------------------------------------------
% register some tokens to be checked for:
\AcroRegisterTrailing . {dot}
\AcroRegisterTrailing - {dash}
\AcroRegisterTrailing \babelhyphen {babel-hyphen}

\acsetup { activate-trailing-tokens = dot }

% some user macros:
\cs_new_protected:Npn \acro_dot:
  { \acro_if_trailing_tokens:nF {dot} {.\@} }

\cs_new_protected:Npn \acro_space:
  { \acro_if_trailing_tokens:nF {dash,babel-hyphen} { \c_space_tl } }

% --------------------------------------------------------------------------
% translations:
% list name
\DeclareAcroTranslation {acronym-list-name}
  {
    Fallback   = Acronyms ,
    English    = Acronyms ,
    French     = Acronymes ,
    German     = Abk\"urzungen ,
    Italian    = Acronimi ,
    Portuguese = Acr\'onimos ,
    Spanish    = Siglas ,
    Catalan    = Sigles ,
    Turkish    = K\i saltmalar
  }

% page name
\DeclareAcroTranslation {acronym-page-name}
  {
    Fallback   = p. ,
    English    = p. ,
    German     = S. ,
    Portuguese = p.
  }

% pages name
\DeclareAcroTranslation {acronym-pages-name}
  {
    Fallback   = pp. ,
    English    = pp. ,
    German     = S. ,
    Portuguese = pp.
  }

% following page
\DeclareAcroTranslation {acronym-next-page}
  {
    Fallback   = f. ,
    English    = f. ,
    German     = f. ,
    Portuguese = s.
  }

% following pages
\DeclareAcroTranslation {acronym-next-pages}
  {
    Fallback   = ff. ,
    English    = ff. ,
    German     = ff. ,
    Portuguese = ss.
  }

\file_input_stop:

